Robust Multiple Description Neural Video Codec with Masked Transformer for Dynamic and Noisy Networks

Multiple Description Coding (MDC) is a promising error-resilient source coding method that is particularly suitable for dynamic networks with multiple (yet noisy and unreliable) paths. However, conventional MDC video codecs suffer from cumbersome architectures, poor scalability, limited loss resilience, and lower compression efficiency. As a result, MDC has never been widely adopted. Inspired by the potential of neural video codecs, this paper rethinks MDC design. We propose a novel MDC video codec, NeuralMDC, demonstrating how bidirectional transformers trained for masked token prediction can vastly simplify the design of MDC video codec. To compress a video, NeuralMDC starts by tokenizing each frame into its latent representation and then splits the latent tokens to create multiple descriptions containing correlated information. Instead of using motion prediction and warping operations, NeuralMDC trains a bidirectional masked transformer to model the spatial-temporal dependencies of latent representations and predict the distribution of the current representation based on the past. The predicted distribution is used to independently entropy code each description and infer any potentially lost tokens. Extensive experiments demonstrate NeuralMDC achieves state-of-the-art loss resilience with minimal sacrifices in compression efficiency, significantly outperforming the best existing residual-coding-based error-resilient neural video codec.

==> tex/91_AAAI_checklist.tex <==
\clearpage
\section{Reproducibility Checklist}
This paper:
\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes)
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes)
    \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (yes)
\end{itemize}

\noindent
Does this paper make theoretical contributions? (no)
\iffalse
\begin{itemize}
    \item All assumptions and restrictions are stated clearly and formally. (yes/partial/no)
\item All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)
\item Proofs of all novel claims are included. (yes/partial/no)
\item Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)
\item Appropriate citations to theoretical tools used are given. (yes/partial/no)
\item All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)
\item All experimental code used to eliminate or disprove claims is included. (yes/no/NA)
\end{itemize}
\fi

\noindent
Does this paper rely on one or more datasets? (yes)
\begin{itemize}
    \item A motivation is given for why the experiments are conducted on the selected datasets (yes)
\item  All novel datasets introduced in this paper are included in a data appendix. (NA)
\item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (NA)
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes)
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes)
\item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (NA)
\end{itemize}

\noindent
Does this paper include computational experiments? (yes)
\begin{itemize}
    \item Any code required for pre-processing data is included in the appendix. (no)
\item All source code required for conducting and analyzing the experiments is included in a code appendix. (no)
\item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes)
\item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes)
\item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes)
\item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes)
\item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes)
\item This paper states the number of algorithm runs used to compute each reported result. (yes)
\item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes)
\item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (no)
\item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes)
\item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (no)
\end{itemize}

==> tex/99_outlines.tex <==
\section{Outlines}
Video streaming over dynamic and lossy networking environments are challenging\todo{cite Wei's multi channel paper}.
Existing neural video codecs are agnostic to underlying networking environments. 
This work is the first to explore utilizing neural network to let the video compression meets the communication networks. make codecs more intelligent and adaptive to network changes.

Networking characteristics: highly dynamic,  high loss ratios, abundant radio resources (multiple channels/paths).

Challenges posing to video codecs:
\begin{itemize}
    \item highly dynamics -> fast bitrate adaption on the fly -> SVC and MDC.
    \item multiple channels -> SVC and MDC.
    \item high loss ratios -> decodable even with loss -> MDC.
\end{itemize}

\hl{nerual MDC: fine-grained rate adaptation; independently decodable; mutually refinable; loss recovery and state mismatch control.}

\hl{We systematically and comprehensively investigate existing various types of neural video codecs and find that video codecs based on masked transformer makes MDC design simple and efficient.}
\begin{itemize}
    \item \textbf{Independently decodable and mutually refinable. Requirements on entropy model: can efficiently estimate the distributions of any portion of latent representation without any side information~\cite{balle2018variational}. }
    \begin{itemize}
        \item splits the latent tensor along the channel dimension for entropy coding is commonly used in existing networks. However, this is mainly used to speed up the coding speed. Existing works~\cite{minnen2020channel, li2022hybrid, he2021checkerboard, xiang2022mimt} sequentially compress each splits to exploit the rich spatial context for better compression efficiency. For MDC, to achieve independently decodable, we need to sacrifice a little bit compression efficiency, and we independently compress each split.
        \item Channel-wise autoregressive entropy models~\cite{minnen2020channel}, which splits the latent tensor along the channel dimension and autoregressive along the channel dimension -> sequentially decodable likes SVC.
        \item We do not consider Implicit Neural Representations -based video codecs~\cite{chen2021nerv}, because it needs to overfit a video and doese not generalize to other videos for general compression purpose without retraining. Besides, the loss of INR model weights cannot be efficiently estimated from received weights.
    \end{itemize}
    
    \item \textbf{Loss Recovery for spatial loss at single frame level. Descriptions are equally important.} No some descriptions are more important than others. \todo{The impact of motion vector~\cite{lu2019dvc} How mv vector can be estimated from received residual vector?. The impact of different contexts~\cite{li2023neural}. How one context can be estimated from received other contexts?}\\ 
    \jiaxiang{DVC: impact of mv loss and residual vector loss.}
    \jiaxiang{Grace: impact of mv loss and residual vector loss.}\\
    \hl{we use single type of context/condition, latent tokens.}
    
    \item state-mismatch control. Loss recovery for temporal loss. 
    \todo{how existing neural video codecs handle the temporal error propagation due to the mismatch of encoder and decoder states? } \wei{literature survey}
\end{itemize}



